MAV Development Towards Navigation in Unknown and Dark Mining Tunnels

The Mining industry considers the deployment of MAV for autonomous inspection of tunnels and shafts to increase safety and productivity. However, mines are challenging and harsh environments that have a direct effect on the degradation of high-end and expensive utilized components over time. Inspired by this effect, this article presents a low cost and modular platform for designing a fully autonomous navigating MAV without requiring any prior information from the surrounding environment. The design of the proposed aerial vehicle can be considered as a consumable platform that can be instantly replaced in case of damage or defect, thus comes into agreement with the vision of mining companies for utilizing stable aerial robots with reasonable cost. In the proposed design, the operator has access to all on-board data, thus increasing the overall customization of the design and the execution of the mine inspection mission. The MAV platform has a software core based on ROS operating on an Aaeon UP-Board, while it is equipped with a sensor suite to accomplish the autonomous navigation equally reliable when compared to high-end and expensive platforms.

==> Tikz/PlayStationEye.tex <==
 \tikzsetnextfilename{PlayStationEye} 
   \begin{tikzpicture}
   %% Images
   \node at (0,0) [align=center] (left1) {\includegraphics[width=\linewidth]  {PScamera1.png}};
    \node[ right= 2 cm of left1,align=center] (middle1) {\includegraphics[width=\linewidth]  {PScamera2.png}};
\node[ right= 2 cm of middle1,align=center] (right1) {\includegraphics[width=\linewidth]  {PScamera3.png}};
   
%% Text

%\node [below= 1.5 cm of left2, align=center] (left3) {\includegraphics[width=\linewidth]  {left3.png}};
%    \node[ right= 2 cm of left3,align=center] (middle3) {\includegraphics[width=\linewidth]  {middle3.png}};
%\node[ right= 2 cm of middle3,align=center] (right3) {\includegraphics[width=\linewidth]  {right3.png}};
\end{tikzpicture}

==> Tikz/ltuPlatform.tex <==
 \tikzsetnextfilename{ltuPlatform} 
 \begin{tikzpicture}
      	\node at (0,0) [align=center] (front) {\includegraphics[width=\linewidth]  {ps4front.png}};
    \node[ right= 2 cm of front,align=center] (top) {\includegraphics[width=\linewidth]  {ps4top.png}};
\node[ right= 2 cm of top,align=center] (bottom) {\includegraphics[width=\linewidth]  {ps4bottom.png}};
        %% Front top bottom view
        %\node at (-1.7,7) [right] {\Huge Front View};
        %\node at (35,7) [right] {\Huge Bottom View};
        %\node at (16.6,7) [right] {\Huge Top View};
        %%GpPro
        \draw[-latex,line width = 0.1cm,white!50!black,dashed] (0,-6.5) -- (-0.2,-3);
	    \node at (-1,-7) [right] {\Huge PS camera};
	    %% Lightbar
        \draw[-latex,line width = 0.1cm,white!50!black,dashed] (-2.5,-5.0) -- (-3.5,-1);
        \node at (-5.5,-5.5) [right] {\Huge LED light bar};
        \draw[-latex,line width = 0.1cm,white!50!black,dashed] (-2.5,-5.0) -- (3.5,-1.4);
        %%Camnera Mount
        \draw[-latex,line width = 0.1cm,white!50!black,dashed] (2.5,-5) -- (0.0,-1.3);
	    \node at (1.7,-5.5) [right] {\Huge Camera Mount};
        %% Sizes
        \draw[latex-latex,line width = 0.1cm,white!50!black,dashed] (14.5,5.5) -- (26,5.5);
        \node at (20.5,6) [] {\Huge 0.35~$\unit{m}$};
        \draw[latex-latex,line width = 0.1cm,white!50!black,dashed] (13.2,3) -- (13.2,-4.5);
        \node at (12.5,0) [rotate=90] {\Huge 0.25~$\unit{m}$};
        %% Lidar
        \draw[-latex,line width = 0.1cm,white!50!black,dashed] (20,-6) -- (20,-4);
	    \node at (18.5,-6.5) [right] {\Huge 2D Lidar};
        %% One beam Lidar
        \draw[-latex,line width = 0.1cm,white!50!black,dashed] (46,0) -- (42.5,0);
	    \node at (46,0) [right] {\Huge Rangefinder};
        %% LED
        \draw[-latex,line width = 0.1cm,white!50!black,dashed] (34.6,0) -- (37.6,0);
	    \node at (32.6,0) [right] {\Huge LED};
        %% Optical Flow
        \draw[-latex,line width = 0.1cm,white!50!black,dashed] (39.9,-6) -- (39.9,0);
	    \node at (38,-6.5) [right] {\Huge Optical-flow};
    \end{tikzpicture}

==> Tikz/opticalflow.tex <==
 \tikzsetnextfilename{opticalflow} 
   \begin{tikzpicture}
   %% Images
   \node at (0,0) [align=center] (left1) {\includegraphics[width=\linewidth]  {optical1.png}};
    \node[ right= 2 cm of left1,align=center] (middle1) {\includegraphics[width=\linewidth]  {optical3.png}};
\node[ right= 2 cm of middle1,align=center] (right1) {\includegraphics[width=\linewidth]  {optical3.png}};
   
%% Text

%\node [below= 1.5 cm of left2, align=center] (left3) {\includegraphics[width=\linewidth]  {left3.png}};
%    \node[ right= 2 cm of left3,align=center] (middle3) {\includegraphics[width=\linewidth]  {middle3.png}};
%\node[ right= 2 cm of middle3,align=center] (right3) {\includegraphics[width=\linewidth]  {right3.png}};
\end{tikzpicture}

==> Tikz/schematic_problem.tex <==
\tikzsetnextfilename{schematic_problem} 
\tikzstyle{block} = [draw,  rectangle, 
    minimum height=2em, minimum width=6em]
    \tikzstyle{hblock} = [draw,  rectangle, 
    minimum height=2em, minimum width=9em]
    \tikzstyle{vblock} = [draw,  rectangle, 
    minimum height=2em, minimum width=4em]
    \tikzstyle{vvblock} = [draw,  rectangle, 
    minimum height=2em, minimum width=4.8em]
\tikzstyle{sblock} = [draw,  rectangle, 
    minimum height=2em, minimum width=6em]
\tikzstyle{blockdash} = [draw,dashed,  rectangle, 
    minimum height=3em, minimum width=6em]
\tikzstyle{input} = [coordinate]
\tikzstyle{output} = [coordinate]
\tikzstyle{pinstyle} = [pin edge={to-,thin,black}]
\begin{tikzpicture}
    % We start by placing the blocks
   % \fill[gray!40!white] (-14,-5) rectangle (-12,-5);
    \node[block, align=center] (Navigation) at (0,0) {Navigation};
    
    \node[block, right= 2 cm of Navigation,align=center] (Controller){Controller};
    \node [ right= 3cm  of Controller,align=center] (MAV) {\includegraphics[width=1cm]{quadcopter.png}};
    \node[hblock, above= 0.22 cm of MAV,align=center] (2D lidar){2D lidar};
    \node[hblock, below= 0.21 cm of MAV,align=center] (Optical Flow){Optical flow \\ One beam lidar};
    \node[draw, vblock, rotate=90, above left = 0.84cm and 0cm  of Optical Flow,align=center,anchor=north] (Flight controller) {Flight \\ controller};
    \node[draw, vvblock, rotate=90,above right =0.84cm and -0.72cm  of Optical Flow,align=center,anchor=north] (Camera) {Camera};
    \node[block, below= 2 cm of Controller,align=center] (State estimation){State estimation};
    \node[block, right= 2.5 cm of MAV,align=center] (Visual processing){Visual feedback};
  %  \node[block, left= 3.5 cm of Visual processing,align=center] (Operator){Operator};
  %  \node[block, above left= 0.0 cm and 0.5cm of Visual processing,align=center] (online){Online};
 %   \node[block, below left= 0.0 cm and 0.5cm of Visual processing,align=center] (offline){Offline};
    %%% connecting nodes
    \node[output,right= 2 cm of MAV ] (cam2ve){};
    \node[output,above = 2.5 cm  of cam2ve ] (cam2nav){};
    \node [above = .8 cm  of 2D lidar ]  () {\pgfuseplotmark{*}};
    \node [output,above = .9 cm  of 2D lidar ]  (2dtonav) {};
    %%% Drawing lines
     \draw [draw,-{Stealth[scale=1.0]}, text width=3cm,align=center] (Navigation) -- node[pos=0.2,above,xshift=0.5cm,yshift=-0.35cm] {\tiny Navigation \\  \tiny commands} (Controller);
     \draw [draw,-{Stealth[scale=1.0]}, text width=3cm,align=center] (Controller) -- node[pos=0.2,above,xshift=0.5cm,yshift=-0.35cm] {\tiny controller \\ commands} (Flight controller);
    % \draw [draw,-{Stealth[scale=1.0]}, text width=4cm,align=center] (Visual processing) |- node[pos=0.4,above,xshift=-0.3cm ] {\tiny Compressed stream} (online);
   %  \draw [draw,-{Stealth[scale=1.0]}, text width=4cm,align=center] (Visual processing) |- node[pos=0.4,below,xshift=-0.3cm ] {\tiny Image stream} (offline);
   %  \draw [draw,-{Stealth[scale=1.0]}, text width=2.5cm,align=center] (online) -| node[pos=0.2,above ] {\tiny \gls{ar}} (Operator);
%     \draw [draw,-{Stealth[scale=1.0]}, text width=2.0cm,align=left] (offline) -| node[pos=0.2,below,xshift=0.3cm] {\tiny 3D model} (Operator);
      \draw [draw,-{Stealth[scale=1.0]}, text width=2.5cm,align=center] (State estimation) -- node[pos=0.2,above ] {} (Controller);
      \draw [-] (Camera) -- node [name=y,pos=0.6,above] {} (cam2ve);
      \draw [-] (cam2ve) -- node [name=y,pos=0.6,above] {} (cam2nav);
       \draw [-] (2D lidar) -- node [name=y,pos=0.6,above] {} (2dtonav);
      \draw [draw,-{Stealth[scale=1.0]}, text width=4cm,align=center] (Optical Flow) |- node[xshift=-1.6cm ] {\tiny range measurement, image stream, IMU measurements} (State estimation);
      \draw [draw,-{Stealth[scale=1.0]}, text width=2.5cm,align=center] (cam2ve) |- node[pos=0.2,above ] {} (Visual processing);
      \draw [draw,-{Stealth[scale=1.0]}, text width=8cm,align=center] (cam2nav) -| node[pos=0.2,above ] {\tiny range measurements, compressed image stream} (Navigation);
    %%%% Textx
    %\node [above right= 0.2 cm and 0.0cm of Navigation,align=center] {\tiny Navigation \\  \tiny commands};
    
    
    
  %  \node[sblock, below= 0.5cm of VGB,align=center] (PF)  {PF};
   %  \node[sblock, right = 0.5cm of VGB,align=center] (Controller){Controller};
%    \node[sblock, right = 0.5cm of Controller,align=center] (Flight Controller){Flight Controller};
%    \node [ above= 0.2cm  of Flight Controller,align=center] (MAV) {\includegraphics[width=1cm]{quadcopter.png}};
%        \node[sblock, right = 0.5cm of Flight Controller,align=center] (Optical Flow){Optical Flow};
 %       \node[sblock, below = 0.5cm of Optical Flow,align=center] (Lidar){Lidar};
 %   \node[sblock, above = 0.5cm of Optical Flow,align=center] (Camera){Camera};
\end{tikzpicture}


